Fully Geometric Panoramic Localization

We introduce a lightweight and accurate localization method that only utilizes the geometry of 2D-3D lines. Given a pre-captured 3D map, our approach localizes a panorama image, taking advantage of the holistic 360 view. The system mitigates potential privacy breaches or domain discrepancies by avoiding trained or hand-crafted visual descriptors. However, as lines alone can be ambiguous, we express distinctive yet compact spatial contexts from relationships between lines, namely the dominant directions of parallel lines and the intersection between non-parallel lines. The resulting representations are efficient in processing time and memory compared to conventional visual descriptor-based methods. Given the groups of dominant line directions and their intersections, we accelerate the search process to test thousands of pose candidates in less than a millisecond without sacrificing accuracy. We empirically show that the proposed 2D-3D matching can localize panoramas for challenging scenes with similar structures, dramatic domain shifts or illumination changes. Our fully geometric approach does not involve extensive parameter tuning or neural network training, making it a practical algorithm that can be readily deployed in the real world. Project page including the code is available through this link: https://82magnolia.github.io/fgpl/.

==> sec/5_experiments.tex <==
\section{Experiments}
\label{sec:exp}

% Implementation details
We evaluate our method on a wide range of localization scenarios and establish comparisons against existing methods.
Our method is implemented in PyTorch~\cite{pytorch}, and we use a single RTX2080 GPU with an Intel Core i7-7500U CPU.
We fix the set of hyperparameters with the inlier threshold $\tau=0.1$, number of query points $|Q|=642$, and number of translations per line map $N_t=500$.
% Despite using a fixed hyperparameter setup, our method performs competitively against existing methods using visual descriptors, and attains robustness even in chaning lighting conditions or large scale scenes.
% Additional details about the implementation are deferred to the supplementary material.

\input{figures/fig_pose_search}
\input{tables/refinement_comparison}

\subsection{Performance Analysis}
\label{seC:perf}
We evaluate our method in Stanford 2D-3D-S~\cite{stanford2d3d} and OmniScenes~\cite{piccolo}, following prior work~\cite{piccolo, cpo, ldl, sphere_cnn, gosma}.
Stanford 2D-3D-S consists of 1413 panoramas captured in 272 rooms, while OmniScenes is a recently proposed dataset that consists of 4121 panoramas from 7 rooms.
% Unlike Stanford 2D-3D-S, OmniScenes contains splits with scene changes occuring between the 3D map building and panorama capture.
Unless specified otherwise, we use the entire Stanford 2D-3D-S dataset and the Extreme split from OmniScenes, which is the most challenging split that contains both scene changes and fast camera motion.

\paragraph{Pose Search Evaluation}
Our pose search can quickly compare the candidate rotations and translations in a 3D map and find the closest pose.
Our approach is compared against neural network-based (SFRS~\cite{openibl}, Cosplace~\cite{cosplace}), color distribution-based (PICCOLO~\cite{piccolo}, CPO~\cite{cpo}) and line-based (LDL~\cite{ldl}, Chamfer~\cite{line_chamfer}) methods.
%We first establish exhaustive comparisons against existing pose search methods, namely neural network-based (SFRS~\cite{openibl}, Cosplace~\cite{cosplace}), color distribution-based (PICCOLO~\cite{piccolo}, CPO~\cite{cpo}) and line-based (LDL~\cite{ldl}, Chamfer~\cite{line_chamfer}) methods.
For implementing these methods we use the colored point cloud from the tested datasets and render synthetic views at various translations and rotations, from which we prepare neural network descriptors.
For fair comparison, we use the identical pool of translations and rotations.
We additionally implement neural network-based methods that take line images as input instead of the original RGB images (SFRS\textsuperscript{L}, Cosplace\textsuperscript{L}), to examine how these methods can handle geometric localization scenarios.
% Further details about the implementations are reported in the supplementary material.

\if 0
We first establish comparisons against existing pose search methods, namely neural network-based~\cite{openibl, cosplace}, color distribution-based~\cite{piccolo, cpo} and line-based~\cite{line_chamfer, ldl} methods.
Neural network-based methods (SFRS~\cite{openibl}, Cosplace~\cite{cosplace}) extract a single feature vector for each query/reference image and retrieve poses in the map with the closest feature vector distances to the query.
For implementing these methods we use the colored point cloud from the tested datasets and render synthetic views at various translations and rotations, from which we prepare neural network descriptors.
Color distribution-based methods (PICCOLO~\cite{piccolo}, CPO~\cite{cpo}) compare the color values in the panorama and those in various locations within the point cloud to retrieve poses with coherent color values between the image and the map.
Unlike the aforementioned methods that exploit the photometric information in 2D and 3D, line-based methods (LDL~\cite{ldl}, Chamfer~\cite{line_chamfer}) solely use lines for pose search, where poses with similar spatial arrangements of lines are retrieved.
We additionally implement neural network-based methods that take line images as input instead of the original RGB images (SFRS\textsuperscript{L}, Cosplace\textsuperscript{L}), to examine how these methods can handle geometric localization scenarios.
Further details about the implementations are reported in the supplementary material.
\fi

Figure~\ref{fig:pose_search} shows the top-1 recall curve and the runtime of all the tested baselines.
Our method attains a high recall even at strict translation and rotation thresholds, and shows a much shorter runtime than neural network-based or color-based methods.
While several line-based methods (LDL, Chamfer) exhibit a shorter runtime, the retrieved poses from there methods are relatively inaccurate compared to our method.
The point distance functions along with the efficient distance function computation enables fast and accurate pose search, where the efficacy of each component is further examined in Section~\ref{sec:ablation}.

\paragraph{Pose Refinement Evaluation}
The candidate pose is further refined by minimizing the distances between matched features.
We compare our pose refinement procedure against three classes of refinement methods: line-based~\cite{line_transformer, gluestick}, point-based~\cite{sarlin2020superglue,lightglue,loftr,piccolo,cpo}, and geometric~\cite{gomatch,bpnp_net,line_refinement}.
While line-based methods and point-based methods find matches using the photometric information near the line segments and points to increase accuracy, geometric methods only rely on the locations of keypoints (GoMatch~\cite{gomatch}, BPnPNet~\cite{bpnp_net}) or lines, as we propose.
We additionally implement the line alignment method proposed from Gao et al.~\cite{line_refinement}, along with a conceived baseline that directly minimizes Equation~\ref{eq:pdf_loss} with gradient descent (PDF minimization).

\if 0
We further compare our pose refinement procedure against three classes of refinement methods: line-based~\cite{line_transformer, gluestick}, point-based~\cite{sarlin2020superglue,lightglue,loftr,piccolo,cpo}, and geometric~\cite{gomatch,bpnp_net,line_refinement}.
Line-based methods and point-based methods utilize the photometric information near the line segments and points to establish matchings in 2D and 3D.
For geometric methods, we first consider methods that learn geometric descriptors for each keypoint (GoMatch~\cite{gomatch}, BPnPNet~\cite{bpnp_net}) and those that take line images as input, similar to the baselines constructed for pose search.
We additionally implement the line alignment method proposed from Gao et al.~\cite{line_refinement}, along with a conceived baseline that directly minimizes Equation~\ref{eq:pdf_loss} with gradient descent (PDF minimization).
\fi

\if 0
We further compare our pose refinement procedure against three classes of refinement methods: line-based~\cite{line_transformer, gluestick}, point-based~\cite{sarlin2020superglue, lightglue, loftr, piccolo, cpo}, and geometric~\cite{gomatch, bpnp_net, line_refinement}.
Line-based methods (Line Transformer~\cite{line_transformer}, Gluestick~\cite{gluestick}) matches line features extracted using neural networks that consume the photometric information near each line segment.
Several point-based methods (SuperGlue~\cite{sarlin2020superglue}, LightGlue~\cite{lightglue}, LoFTR~\cite{loftr}) also follow a similar approach but for points, while others (PICCOLO~\cite{piccolo}, CPO~\cite{cpo}) directly match the color values in 2D and 3D without using neural networks.
For geometric methods, we first consider methods that learn geometric descriptors for each keypoint (GoMatch~\cite{gomatch}, BPnPNet~\cite{bpnp_net}) and those that take line images as input, similar to the baselines constructed for pose search.
We additionally implement the line alignment method proposed from Gao et al.~\cite{line_refinement}, along with a conceived baseline that directly minimizes Equation~\ref{eq:pdf_loss} with gradient descent (PDF minimization).
\fi

Table~\ref{table:pose_refine} shows the localization accuracy at varying accuracy thresholds.
Here we first retrieve the same top-1 pose using our pose search scheme, and perform refinement using the aforementioned methods.
Our method consistently outperforms all the tested geometric methods, while showing competitive performance against line-based and point-based refinement methods that use visual descriptors.
Note the accuracy gap between the best performing visual descriptor-based method (LightGlue) and our method is on average around 10\%.
Such results suggest the effectiveness of using line intersections for refinement along with the disambiguation from principal directions.

\paragraph{Robustness to Lighting Changes}
We finally investigate the robustness of our method amidst lighting changes, and establish comparisons against existing methods.
Specifically, we separately measure the performance of pose search and refinement after applying synthetic color variations to the input panorama, similar to the experiments conducted in LDL~\cite{ldl}.
Here we consider three types of color variations (intensity, gamma, and white balance), where we apply two levels of variations for each type, totalling six variations.
Additional details about the setup are reported in the supplementary material.

Table~\ref{table:lighting_refine} displays the pose refinement performance at varying lighting conditions, where all the tested methods take the top-1 pose search results using our method as input.
Our refinement scheme performs competitively against visual descriptor-based methods, while showing a much smaller range and standard deviations in localization accuracy.
A similar trend is observable in Figure~\ref{fig:lighting_pose_search}, where we report the recall curves of top-1 retrievals from various pose search methods.
The size of the shaded regions, which indicates the range of recall values under illumination changes, is much smaller for our method compared to the baselines.
By using lines and their intersections as the only cues for localization, our method can remain robust against lighting condition changes.
\input{tables/lighting_refine}

\input{figures/fig_lighting_pose_search}
\subsection{Large-scale Localization}
We evaluate our method in large-scale localization scenarios, where the geometric methods as ours can benefit from the speed and the lightweight map representations.
Here we conjoin multiple room-level line maps in OmniScenes~\cite{piccolo} and Stanford 2D-3D-S~\cite{stanford2d3d} to create four large-scale maps: \textit{split 1 }containing all rooms in OmniScenes, \textit{split 2} containing all rooms in Area 1 from Stanford 2D-3D-S, \textit{split 3} and \textit{split 4} containing 40 and 60 office rooms in Stanford 2D-3D-S respectively.
An exemplary large scale map is shown in Figure~\ref{fig:overview}.

Table~\ref{table:large_scale} shows the localization results, where we compare  against LDL~\cite{ldl} and various combinations of neural network-based pose search and refinement methods.
Note that for baselines other than LDL, we use the information from the colored point cloud to extract descriptors.
Our method largely outperforms LDL and demonstrates competitive performance against neural network-based methods.
Further, due to the efficient pose search scheme proposed in Section~\ref{sec:pose_search}, our method exhibits an order-of-magnitude shorter search time compared to the baselines.
In addition, as our method only requires the 3D distance function values to be stored prior to localization, the map size is much smaller than the baselines that additionally cache global/local feature descriptors.
We make a detailed analysis of the map size in the supplementary material.

% Table 3
\input{tables/large_scale}
\input{tables/ablation_search}
\input{tables/ablation_refine}

\subsection{Ablation Study}
\label{sec:ablation}
\paragraph{Pose Search}
We first ablate the key constituents of the pose search pipeline using the entire Area 1 of Stanford 2D-3D-S~\cite{stanford2d3d}.
Here we report the localization error and runtime for top-1 retrieval.
Table~\ref{table:ablation_search}\textcolor{red}{a} suggests that using point distance functions along with line distance functions enhance localization performance.
Note that by comparing with Table~\ref{table:large_scale}, there's a performance gap between using line distance functions with large number of query points ($|Q|=642$) as in our method and LDL that uses fewer points ($|Q|=42$).
Due to the efficient distance function comparison, our method can seamlessly handle large number of query points during pose search, which would lead to excessive memory and runtime consumption for LDL.
Table~\ref{table:ablation_search}\textcolor{red}{b},~\ref{table:ablation_search}\textcolor{red}{c} further supports this claim: decoupling rotation/translation for 3D distance functions and interpolating and canonicalizing 2D distance functions lead to significant runtime drops, while showing almost no loss in accuracy.

% Table 5, Figure 7

\paragraph{Pose Refinement}
We further ablate key components of pose refinement using Room 2 from OmniScenes~\cite{piccolo}.
Table~\ref{table:abl_refine} displays the localization accuracy and the median translation/rotation errors.
Only optimizing translation leads to larger rotation errors, which suggests the importance of rotation refinement.
In addition, directly performing nearest neighbor matching without using intersection clusters lead to a large drop in localization performance.
As intersection clusters prevent outlier matches, they are crucial for accurate pose refinement.
We conduct further ablation experiments in the supplementary material.


% Table 6

\paragraph{Applicability to Floorplan Localization}
% Table 4
\input{tables/layout_localization}
While our method is originally designed for localizing against 3D line maps obtained from point cloud scans or structure from motion, we find that our fully geometric setup is versatile to handle 3D floorplan maps without any changes in the hyperparameter configuration.
Following prior works~\cite{lalaloc,lalaloc++,laser2d}, we test our method on localizing panoramas against 3D lines extracted from a floorplan map, where additional details about the data preparation process is explained in the supplementary material.
We use the Structured3D~\cite{Structured3D} dataset for evaluation.
As the lines directly extracted from panoramas are not compatible with the 3D floorplan maps, we instead use the lines from 2D layout annotations.
Despite using this additional information, Table~\ref{table:layout_localization} shows that our method can outperform existing methods.
Further, unlike prior works that only estimate the 2D translation and rotation, our method can estimate the full 6DoF pose while attaining competitive accuracy.
Therefore, if combined with sufficiently accurate 2D layout extraction from panoramas (removing the demand for 2D layout annotations), we expect our method to perform practical floorplan localization.


